Learning to bid in revenue-maximizing auctions

We consider the problem of the optimization of bidding strategies in prior-dependent revenue-maximizing auctions, when the seller fixes the reserve prices based on the bid distributions. Our study is done in the setting where one bidder is strategic. Using a variational approach, we study the complexity of the original objective and we introduce a relaxation of the objective functional in order to use gradient descent methods. Our approach is simple, general and can be applied to various value distributions and revenue-maximizing mechanisms. The new strategies we derive yield massive uplifts compared to the traditional truthfully bidding strategy.

==> completeKKT.tex <==
\section{Proof of Theorem \ref{thm:kktInH1}}
\subsection{Reminders on the Karush-Kuhn-Tucker conditions}
We first recall the standard KKT conditions in a finite dimensional space: if we try to 
$$
\max_x f(x) \text{ s.t } g_i(x)\leq 0\;, 1\leq i \leq m\;, e_j(x)=0\;, 1\leq j \leq K
$$
if $\lambda_i$ are Lagrange/KKT multipliers, we have at the optimum 
$$
\grad f(x^*)=\sum_{i=1}^m \mu_i^* \grad g_i(x^*)+\sum_{j=1}^K \kappa_j^* \grad e_j(x^*)=0\;.
$$
and by complementary slackness 
$$
\mu_i^* g_i(x^*)=0 \forall i\;.
$$
Recall also that we need $\mu_i^*\geq 0$ but no constraint on $\kappa_j^*$. This are necessary conditions. 

Many results extend the KKT conditions to infinite dimensional spaces with either finitely many or infinitely many variables. See for instance \cite{Clarke1976NewApproachLagrangeMultipliers,ekeland1979,GuignardKKTBanach69}. We rely on \cite{TapiaTrossetKKTInfiniteDim94} who generalize the standard KKT formulation to Hilbert spaces. Somewhat unfortunately, this introduces a heavy load of technical requirements. 

Effectively Proposition 2.2 and Theorem 2.4 generalize the standard KKT conditions. In particular, as compared to the standard formulation the multipliers are replaced by (totally) finite measures.

We will work in the Sobolev space $H^1[0,r]$ which are functions $\gamma$ such that $\gamma$ and $\gamma'$ are in $L^2[0,r]$ (see \cite{TapiaTrossetKKTInfiniteDim94} p.13 and references therein for more information about $H^1$). $H^1$ is a Hilbert space, with the dot product $(\gamma,\nu)_{H^1}=\int_{[0,r]} \gamma(x) \nu(x) dx+\int_{[0,r]} \gamma'(x)\nu'(x) dx$. 

To avoid a number of issues arising in connection with making explicit the gradient in $H^1$ of the functionals we consider, we will work throughout with the variation, i.e. the evaluation of the gradient in a certain direction. 



\subsection{Our problem}
Let's call $r$ the current reserve price. It could be e.g. the monopoly price. We call 
$$
h_\beta(x)=\beta(x)-\beta'(x)\frac{1-F(x)}{f(x)}=\psi_B(\beta(x))\;.
$$
We note as before that $f(x)h_\beta(x)=(\beta(x)(F(x)-1))'$. 

We want to find a strategy $\beta$ (which is increasing and continuous, say) such that we 
$$
\max_\beta \Expb{(X-\psi_B(\beta(X)))G(\beta(X))\indicator{X\geq 0}}
$$
under the constraints that 
\begin{gather*}
\forall r_0\leq r, \Expb{\psi_B(\beta(X))G(\beta(X))\indicator{r_0\leq X\leq r}}\leq 0 \\
\Expb{\psi_B(\beta(X))G(\beta(X))\indicator{0\leq X\leq r}}=0\;.
\end{gather*}
Let's limit ourselves to bidding truthfully beyond $r$. Then we effectively need to maximize 
$$
\max_\beta F(\beta)=\Expb{(X-h_\beta(X))G(\beta(X))\indicator{0\leq X\leq r}}\;.
$$
with the constraints that $\beta(r)=r$. That's the continuity constraint. We can rewrite our constraints as 
$$
\mathfrak{g}_{r_0}(\beta)=-\Expb{\psi_B(\beta(X))G(\beta(X))\indicator{0\leq X\leq r_0}}=-\Expb{h_\beta(X)G(\beta(X))\indicator{0\leq X\leq r_0}}\;.
$$
with the constraint $\mathfrak{g}_{r}(\beta)=0$. 

Now we turn to compute our directional derivatives/gradients to be able to explicit the first order conditions, i.e. the equivalent of the Karush-Kuhn-Tucker conditions in our context
. 
In the next few subsections we will show the following result.
\begin{theorem}\label{thm:FirstOrderConditionsInKKT}
To cancel the generalized Lagrangian, the first order conditions evaluated in the direction of the function $\rho$, (i.e. considering the limit of the functionals of interest at $\beta+t\rho$ as $t\tendsto 0$ in our problem) give	
\begin{align}\label{eq:KKTCdtionsOptInThm}
&\Expb{\indicator{0\leq X\leq r}X\rho(X)g(\beta(X))}
\\&=\Expb{\left[h_\rho(X)G(\beta(X))+h_\beta(X)\rho(X)g(\beta(X))\right]\indicator{0\leq X\leq r}\left(1- \int_X^r\lambda(r_0) dr_0\right)}\notag \\
&+\kappa^* \left\{\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\right\}
\end{align}	
Calling $\Lambda(x)=1-\int_x^r \lambda(y)dy$, this can be rewritten as 
\begin{equation}\label{eq:KKTCdtionsFinalInThm}
\begin{aligned}
&\Expb{\rho(X)\indicator{0\leq X\leq r}g(\beta(X))\left[X-(\Lambda(X)+\kappa^*)\beta(X)\right]}=\\
&\Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]\indicator{0\leq X\leq r}}-\left. G(\beta(x))(1-F(x))(\Lambda(x)+\kappa^*)\rho(x)\right|_0^r\;.
\end{aligned}
\end{equation}

\end{theorem}


\subsection{Gradient computation for equality constraint}

Recall the equality constraint $C_\beta=\Expb{h_\beta(X)G(\beta(X))\indicator{0\leq X\leq r}}=0$. Taking its derivative when $\beta_t=\beta+t\rho$ gives 
\begin{align*}
\frac{\partial}{\partial t}C_{\beta_t}&=\Expb{\indicator{0\leq X\leq r}\rho(X)\left[G(\beta(X))+h_\beta(X)g(\beta(X))\right]}
\\&-\Expb{\indicator{0\leq X\leq r}\rho'(X)\frac{1-F(X)}{f(X)}G(\beta(X))}
\end{align*}Using integration by parts trick (see below for more details) we get 
\begin{gather*}
-\Expb{\indicator{0\leq X\leq r}\rho'(X)\frac{1-F(X)}{f(X)}G(\beta(X))}=\\
\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r-\Expb{\rho(X)[G(\beta(X))+(h_\beta-\beta(X))g(\beta(X))\indicator{0\leq X\leq r}}
\end{gather*}
So that 
\begin{align*}
\frac{\partial}{\partial t}C_{\beta_t}&=\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\;,\\
&=\rho(0)G(\beta(0))+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\;.
\end{align*}



\subsection{Gradient computations and dealing with inequality constraints}

Recall that if $\beta_t=\beta+t\rho$, 
$$
h_{\beta_t}=h_\beta+t h_\rho\;.
$$

So 
$$
\frac{\partial}{\partial t} F(\beta_t)=\Expb{\indicator{0\leq r}[-h_\rho G(\beta(X))+(X-h_\beta(X))\rho(X)g(\beta(X))]}\;.
$$
Also, 
$$
\frac{\partial}{\partial t} \mathfrak{g}_{r_0}(\beta_t)=-\int_0^{r_0} \left[h_\rho(x)G(\beta(x))+h_\beta(x)\rho(x)g(\beta(x))\right]f(x)dx\;.
$$
On the other hand, using \cite{TapiaTrossetKKTInfiniteDim94} we replace the sum of the gradient of the multipliers in the classical formulation by an integral. Let  $\lambda(r_0)$ the Lagrange multiplier associated with $r_0$. 

We have, as analog of the sum of the gradients in the discrete case,
\begin{align*}
\int_0^r \lambda(r_0) \frac{\partial}{\partial t} \mathfrak{g}_{r_0}(\beta_t)dr_0&=-\int_0^r\int_0^r\lambda(r_0)dr_0 [h_\rho(x)G(\beta(x))
\\&+h_\beta(x)\rho(x)g(\beta(x))]f(x)dx\\
&=-\int_0^r [h_\rho(x)G(\beta(x))
\\&+h_\beta(x)\rho(x)g(\beta(x))]f(x)\left(\int_x^r\lambda(r_0) dr_0\right)dx\;.
\end{align*}
Hence to have the generalized Lagrangian equal to zero, the first order conditions give 
\begin{gather*}
-\Expb{\left[h_\rho(X)G(\beta(X))+h_\beta(X)\rho(X)g(\beta(X))\right]\indicator{0\leq X\leq r}\left(\int_X^r\lambda(r_0) dr_0\right)}\\
+\kappa^* \left\{\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\right\}\\
=\\
\Expb{\indicator{0\leq X\leq r}X\rho(X)g(\beta(X))}-\Expb{\indicator{0\leq X\leq  r}[h_\rho G(\beta(X))+h_\beta(X)\rho(X)g(\beta(X))]}
\end{gather*}

This can be rewritten as 
\begin{align}\label{eq:KKTCdtionsOpt}
&\Expb{\indicator{0\leq X\leq r}X\rho(X)g(\beta(X))}
\\&=\Expb{\left[h_\rho(X)G(\beta(X))+h_\beta(X)\rho(X)g(\beta(X))\right]\indicator{0\leq X\leq r}\left(1- \int_X^r\lambda(r_0) dr_0\right)}\notag \\
&+\kappa^* \left\{\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\right\}
\end{align}
This shows Theorem \ref{thm:FirstOrderConditionsInKKT}.

Let us now simplify this expression. 
Let us work on the top part of the right hand side. We're going to use integration by parts again to simplify the expression. 
Let's call 
$$
\Lambda(x)=1-\int_x^r \lambda(y)dy\;.
$$
Note that $\Lambda'(x)=\lambda(x)$. Let 
\begin{align*}
\Gamma&=\Expb{G(\beta(X))h_\rho(X)\Lambda(X)\indicator{0\leq X \leq r}}\\
&=\Expb{G(\beta(X))\rho(X)\Lambda(X)\indicator{0\leq X \leq r}}-\int_0^r G(\beta(x))\rho'(x)(1-F(x))\Lambda(x)dx
\end{align*}
Using integration by parts, we have
\begin{gather*}
\int_0^r G(\beta(x))\rho'(x)(1-F(x))\Lambda(x)dx=\left. G(\beta(x))(1-F(x))\Lambda(x)\rho(x)\right|_0^r - \\
\int_0^r \rho(x)[\beta'(x)g(\beta(x))(1-F(x))\Lambda(x)-
\\f(x)G(\beta(x))\Lambda(x)+G(\beta(x))(1-F(x))\lambda(x)]dx\\
=\left. G(\beta(x))(1-F(x))\Lambda(x)\rho(x)\right|_0^r+\Expb{\rho(X)G(\beta(X))\Lambda(X)\indicator{0\leq X\leq r}}\\
-\Expb{\rho(X)g(\beta(X))\beta'(X)\frac{1-F(X)}{f(X)}\Lambda(X)\indicator{0\leq X\leq r}}-\Expb{\rho(X)G(\beta(X))\frac{1-F(X)}{f(X)}\lambda(X)\indicator{0\leq X\leq r}}
\end{gather*}
Of course, 
$$
-\beta'(x)\frac{1-F(x)}{f(x)}=h_\beta(x)-\beta(x)\text{ and } -\frac{1-F(x)}{f(x)}=\psi_F(x)-x\;.
$$
Hence, 
\begin{gather*}
\int_0^r G(\beta(x))\rho'(x)(1-F(x))\Lambda(x)dx
\\=\left. G(\beta(x))(1-F(x))\Lambda(x)\rho(x)\right|_0^r
+\Expb{\rho(X)G(\beta(X))\Lambda(X)\indicator{0\leq X\leq r}}\\
+\Expb{g(\beta(X))\rho(X)\Lambda(x)\indicator{0\leq X\leq r}(h_\beta(X)-\beta(X))}
\\+
\Expb{\lambda(X)\rho(X)G(\beta(X)))\left[\psi_F(X)-X\right]\indicator{0\leq X\leq r}}\;.
\end{gather*}
We conclude that 
\begin{gather*}
\Gamma=\notag\\
\Expb{\rho(X)g(\beta(X))\Lambda(X)\indicator{0\leq X\leq r}[\beta(X)-h_\beta(X)]}+
\Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]\indicator{0\leq X\leq r}}
\\-\left. G(\beta(x))(1-F(x))\Lambda(x)\rho(x)\right|_0^r
\end{gather*}
% \subsection{Equality constraint}
% \textbf{Adding the equality constraint}
% Recall the equality constraint $C_\beta=\Expb{h_\beta(X)G(\beta(X))\indicator{0\leq X\leq r}}=0$. Taking its derivative when $\beta_t=\beta+t\rho$ gives
% $$
% \frac{\partial}{\partial t}C_{\beta_t}=\Expb{\indicator{0\leq X\leq r}\rho(X)\left[G(\beta(X))+h_\beta(X)g(\beta(X))\right]}-\Expb{\indicator{0\leq X\leq r}\rho'(X)\frac{1-F(X)}{f(X)}G(\beta(X))}
% $$
% Using the same integration by parts trick as before we get
% \begin{gather*}
% -\Expb{\indicator{0\leq X\leq r}\rho'(X)\frac{1-F(X)}{f(X)}G(\beta(X))}=\\
% \left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r-\Expb{\rho(X)[G(\beta(X))+(h_\beta-\beta(X))g(\beta(X))\indicator{0\leq X\leq r}}
% \end{gather*}
% So that
% \begin{align*}
% \frac{\partial}{\partial t}C_{\beta_t}&=\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\;,\\
% &=\rho(0)G(\beta(0))+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\;.
% \end{align*}
% So adding this constraint, the optimality conditions become
\subsection{Putting everything together}
With our new notations, Equation \eqref{eq:KKTCdtionsOpt} reads 
\begin{align*}
\Expb{\indicator{0\leq X\leq r}X\rho(X)g(\beta(X))}=\Gamma+\Expb{\left[h_\beta(X)\rho(X)g(\beta(X))\right]\indicator{0\leq X\leq r}\Lambda(X)}\notag \\
+\kappa^* \left\{\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\right\}
\end{align*}

Using our integration by parts results, Equation \eqref{eq:KKTCdtionsOpt} becomes
\begin{gather*}
\Expb{\rho(X)\indicator{0\leq X\leq r}g(\beta(X))\left[X-\Lambda(X)\beta(X)\right]}
=\\
\Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]\indicator{0\leq X\leq r}}-\left. G(\beta(x))(1-F(x))\Lambda(x)\rho(x)\right|_0^r\\
+\kappa^* \left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\kappa^*\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}
\end{gather*}
or 
\begin{equation}\label{eq:KKTCdtionsFinal}
\boxed{
\begin{aligned}
&\Expb{\rho(X)\indicator{0\leq X\leq r}g(\beta(X))\left[X-(\Lambda(X)+\kappa^*)\beta(X)\right]}=\\
&\Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]\indicator{0\leq X\leq r}}-\left. G(\beta(x))(1-F(x))(\Lambda(x)+\kappa^*)\rho(x)\right|_0^r
\end{aligned}
}
\end{equation}
\subsection{Exploiting Equation \eqref{eq:KKTCdtionsFinal}}
\textbf{Continuity of bid function and implication} We want the bid function to be continuous that requires $\rho(r)=0$. Hence 
$$
-\left. G(\beta(x))(1-F(x))(\Lambda(x)+\kappa^*)\rho(x)\right|_0^r=G(\beta(0))(\Lambda(0)+\kappa^*)\rho(0)
$$


\textbf{Setting the value for $\kappa^*$}
It is rather clear we will take $\kappa^*=-\Lambda(0)$. Indeed this cancels the term in $G(\beta(0))(\Lambda(0)+\kappa^*)\rho(0)$ no matter what the value of $\rho(0)$ is. \\

Now to guarantee equality in Equation \eqref{eq:KKTCdtionsFinal} we can just equate the terms under the expectations. 
This gives the differential representation for our Lagrange/KKT multipliers
$$
\lambda(x)=\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\left[x-(\Lambda(x)-\Lambda(0))\beta(x)\right]\;.
$$
Note that $\Lambda(x)-\Lambda(0)=\int_0^x \lambda(y)dy$.
In other words, we need to solve for $\lambda$ such that
\begin{equation}\label{eq:ODEForlamdbas}
\boxed{
\lambda(x)=\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\left[x-\beta(x)\int_0^x \lambda(y)dy\right]\;.
}
\end{equation}
That would guarantee that the optimality conditions are satisfied. Since $\lambda=\Lambda'$, this is nothing but a first order ODE in $\Lambda$.



\subsubsection{Can we have $\lambda=0$ on an interval?}
Recall that by complimentary slackness this would mean that the seller revenue is not equal to zero on that interval. This implies that $L$ is constant on that interval.  Going back to Equation \eqref{eq:ODEForlamdbas} we see that this implies that $\beta(x)=x/d$, where $d=L(a)=L(b)>0$ is a positive constant on this interval, provided $g(\beta(x))\neq 0$. Note that this implies that $h_\beta(x)=\psi_F(x)/d<0$ on this interval under our assumptions on $\psi_F$. 

Now when $\beta$ is in $H^1$, the seller revenue on $[t,r]$ is a continuous function of $t$. The fact that $h_\beta<0$ on the interval implies that the seller revenue is strictly decreasing on $[a,b]$. \redtext{What follows is quick and may be false. Needs review} So my continuity, we can find $a'<a$ such that the revenue of the seller is non-zero on $[a',b]$ and hence $\lambda=0$ on [a',b]. This ``implies??'', by complimentary slackness, this is the case on $[0,b]$. And this rules out the possibly that $\beta$ be feasible.

\subsubsection{On the solutions of Equation \eqref{eq:ODEForlamdbas} and its solution 
for the thresholded virtual value}
And indeed, this is just a first order differential equation in 
$$
L(x)=\int_0^x \lambda(y)dy\;.
$$
Looking at the equation it's clear that if we can solve it, $\lambda$ is pretty much gonna be positive...
The first order ODE reads
$$
L'(x)=\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\left[x-\beta(x)L(x)\right]\;.
$$
We note further that for the thresholded virtual value, 
$$
\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\beta(x)=\frac{g(\beta(x))}{G(\beta(x))}\beta'(x)=\left[\log G(\beta(x))\right]'
$$
so the equation reads 
$$
L'(x)=m(x)-\left[\log G(\beta(x))\right]' L(x)\;.
$$
The generic solution of this equation is 
$$
L(x)=\frac{C(x)}{G(\beta(x))} 
$$
where 
$$
C'(x)=m(x)G(\beta(x))=xg(\beta(x))\frac{f(x)}{1-F(x)}\;.
$$
Note we are interested in the particular solution that has $L(0)=0$. Calling
$$
C_0(x)=\int_0^x yg(\beta(y))\frac{f(y)}{1-F(y)}dy\;,
$$
we are interested in the solution
$$
\boxed{
\mathfrak{L}(x)=\frac{C_0(x)}{G(\beta(x))}\;.
}
$$
We see that if ${x-\mathfrak{L}(x)\beta(x)}\neq 0$
$$
\frac{\mathfrak{L}'(x)}{x-\mathfrak{L}(x)\beta(x)}=\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\;.
$$


\subsubsection{The case of the function $\beta^*(x)=r(1-F(r))/(1-F(x))$}

% \subsection{Putting things together}
% With our current notations, we have at the optimum according to Equation \eqref{eq:KKTCdtionsOpt}~ \textcolor{red}{if we exclude the last equality constraint}:
% $$
% \Expb{\indicator{0\leq X\leq r}X\rho(X)g(\beta(X))}=\Gamma+\Expb{h_\beta(X)\rho(X)g(\beta(X))\indicator{0\leq X\leq r}\Lambda(X)}
% $$
% Using the alternative representation of $\Gamma$ we have obtained, we get that the right hand side is just
% $$
% \Expb{\beta(X)\rho(X)g(\beta(X))\Lambda(X)\indicator{0\leq X\leq r}}+
% \Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]}
% -\left. G(\beta(x))(1-F(x))\Lambda(x)\rho(x)\right|_0^r
% $$
% \textbf{Bringing constraints in}\\
% The continuity constraint requires that $\rho(r)=0$ for we want $\beta_t(r)=r$ for all $t$ and $\rho$'s.
%
% Hence the optimality conditions \textcolor{red}{(excluding the equality constraint)} become
% \begin{gather*}
% \Expb{\rho(X)\indicator{0\leq X\leq r}g(\beta(X))\left[X-\Lambda(X)\beta(X)\right]}
% =\\
% \Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]}+G(\beta(0))\Lambda(0)\rho(0)\;.
% \end{gather*}
% \textbf{Why we can't ignore the equality constraint}\\
% It is tempting to ``require" that $\Lambda(0)=0$ which means that the $\lambda(x)$ is a probability density...
% Then we could simply require
% $$
% \boxed{
% \lambda(x)=\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\left[x-\Lambda(x)\beta(x)\right]\;.
% }
% $$
% That would guarantee that the optimality conditions are satisfied. Since $\lambda=\Lambda'$, this is nothing but a first order ODE in $\Lambda$. \textcolor{red}{However there's a slight problem; by construction we also need $\Lambda(r)=1$!!! So that's two equality constraints on $\Lambda$ and it won't work in general}


% \textbf{Adding the equality constraint}
% Recall the equality constraint $C_\beta=\Expb{h_\beta(X)G(\beta(X))\indicator{0\leq X\leq r}}=0$. Taking its derivative when $\beta_t=\beta+t\rho$ gives
% $$
% \frac{\partial}{\partial t}C_{\beta_t}=\Expb{\indicator{0\leq X\leq r}\rho(X)\left[G(\beta(X))+h_\beta(X)g(\beta(X))\right]}-\Expb{\indicator{0\leq X\leq r}\rho'(X)\frac{1-F(X)}{f(X)}G(\beta(X))}
% $$
% Using the same integration by parts trick as before we get
% \begin{gather*}
% -\Expb{\indicator{0\leq X\leq r}\rho'(X)\frac{1-F(X)}{f(X)}G(\beta(X))}=\\
% \left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r-\Expb{\rho(X)[G(\beta(X))+(h_\beta-\beta(X))g(\beta(X))\indicator{0\leq X\leq r}}
% \end{gather*}
% So that
% \begin{align*}
% \frac{\partial}{\partial t}C_{\beta_t}&=\left. \rho(x)(F(x)-1)G(\beta(x))\right|_0^r+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\;,\\
% &=\rho(0)G(\beta(0))+\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}\;.
% \end{align*}
% So adding this constraint, the optimality conditions become
% \begin{gather*}
% \Expb{\rho(X)\indicator{0\leq X\leq r}g(\beta(X))\left[X-\Lambda(X)\beta(X)\right]}
% =\\
% \Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]}+G(\beta(0))\Lambda(0)\rho(0)\\
% +\kappa^* \rho(0)G(\beta(0))+\kappa^*\Expb{\rho(X)\beta(X)g(\beta(X))\indicator{0\leq X\leq r}}
% \end{gather*}
% or
% \begin{gather*}
% \Expb{\rho(X)\indicator{0\leq X\leq r}g(\beta(X))\left[X-(\Lambda(X)+\kappa^*)\beta(X)\right]}=\\
% \Expb{\rho(X)G(\beta(X)))\lambda(X)\left[X-\psi_F(X)\right]}+G(\beta(0))(\Lambda(0)+\kappa^*)\rho(0)
% \end{gather*}
% It is rather clear we will take $\kappa^*=-\Lambda(0)$.
% Proceeding as above we get the differential representation
% $$
% \lambda(x)=\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\left[x-(\Lambda(x)-\Lambda(0))\beta(x)\right]\;.
% $$
% Note that $\Lambda(x)-\Lambda(0)=\int_0^x \lambda(y)dy$.
% In other words, we need to solve for $\lambda$ such that
% $$
% \boxed{
% \lambda(x)=\frac{g(\beta(x))}{G(\beta(x))}\frac{f(x)}{1-F(x)}\left[x-\beta(x)\int_0^x \lambda(y)dy\right]\;.
% }
% $$

\textbf{Why that means local optimality for thresholded virtual value}
Suppose we're given a candidate for local optimality $\beta$. So if $g>0$ on the support of $\beta$ and if $f>0$, we would have $\lambda(x)>0$ everywhere (assuming the bracket is positive). In this case by complementary slackness, we would have 
$$
\forall 0\leq r_0 \leq r \;, \; \mathfrak{g}_{r_0}(\beta^*)=0=-\Expb{\psi_B(\beta^*(X)) G(\beta^*(X)) \indicator{0\leq X\leq r_0}}\;.
$$ 
Which would imply that 
$$
\psi_B(\beta^*(x))G(\beta^*(x))=0 \; \forall 0\leq x \leq r_0\;.
$$
Actually it should be almost surely but with continuity it implies everywhere.
So long story short: if we can show $\lambda>0$ when $\beta$ is thresholded virtual value, then thresholding is locally optimal. 


\subsection{Conclusion}
%That would suggest that \textbf{thresholding the virtual value is locally optimal}. 

The only thing to verify is that with $\beta(x)=\frac{r(1-F(r))}{1-F(x)}$, we can pick $\lambda\geq 0$ that solves the above Equation \eqref{eq:ODEForlamdbas}. That would show local optimality it seems. 



\subsubsection{General case with $\beta^*$ and $r$ monopoly price}
Recall that to show that $\lambda(x)>0$ we need to verify
$$
\mathfrak{L}'(x)> 0
$$
which amounts to showing that 
$$
x-\mathfrak{L}(x)\beta(x)>0\; \text{ on } (0,r) \text{ when }\beta(x)=\frac{r(1-F(r))}{1-F(x)}\;.
$$


The condition 
$$
x-\mathfrak{L}(x)\beta(x)>0\; \text{ on } (0,r) \text{ when }\beta(x)=\frac{r(1-F(r))}{1-F(x)}
$$
reads alternatively, based on the work done above, 
$$
xG(\beta(x))>C_0(x)\beta(x)=\beta(x)\int_0^x yg(\beta(y))\frac{f(y)}{1-F(y)}dy \;, \forall 0<x<r\;.
$$
With $\beta(x)=r(1-F(r))/(1-F(x))$, we have 
\begin{align*}
\beta(x)\int_0^x yg(\beta(y))\frac{f(y)}{1-F(y)}dy&=\frac{r(1-F(r))}{1-F(x)}\int_0^x yg(\beta(y))(1-F(y))\frac{\beta'(y)}{r(1-F(r))}dy\\ 
&=\frac{1}{1-F(x)}\int_0^x yg(\beta(y))(1-F(y))\beta'(y)dy \\
&=\frac{1}{1-F(x)}\left[\left.xG(\beta(x))(1-F(x))\right|_0^r+\int_0^x G(\beta(x))f(x)\psi_F(x)dx \right]\\
&=xG(\beta(x))+\frac{1}{1-F(x)}\int_0^x G(\beta(x))f(x)\psi_F(x)dx\;.
\end{align*}
Hence our condition 
$x-\mathfrak{L}(x)\beta(x)>0\; \text{ on } (0,r) \text{ when }\beta(x)=\frac{r(1-F(r))}{1-F(x)}$
now reads 
$$
\boxed{\int_0^x G(\beta(x))f(x)\psi_F(x)dx<0 \;, \forall 0<x<r\;.}
$$
And that is obviously true for $r$ the monopoly price... since $\psi_F<0$ below it!!!

\textcolor{red}{We should look back at the optimality conditions at the optimal $r^*$ and see if things check out there too. We have a bit of leeway on the integral. If the optimality conditions we have back then are $\Expb{G(\beta(X))\psi_F(X)\indicator{0\leq X\leq r^*}}=0$ we're in business}

Note that we have shown that 
$$
\beta(x)C_0(x)=xG(\beta(x))+\Expb{G(\beta(X))\psi_F(X)|X<x}
$$
and hence 
$$
\mathfrak{L}(x)=\frac{x}{\beta(x)}+\frac{\Expb{G(\beta(X))\psi_F(X)|X<x}}{\beta(x)G(\beta(x))}\;.
$$
Not clear it's so helpful...


==> fullOldKKTAttempts.tex <==
\newpage
\section{Formal proof KKT}
\redtext{Still experimental!!}\\
Some of the tools we might need could be in \cite{TapiaTrossetKKTInfiniteDim94,GuignardKKTBanach69}.

Roughly speaking the idea is to try to show that thresholding is locally optimal as an extension of any bidding strategy whose reserve value is $r$. That's the context of the computations shown above. 

So then we have to solve the infinite programming problem 
\begin{gather*}
\max F(\beta)=\Expb{[X-h_\beta(X)]G\beta(X)\indicator{0\leq X\leq r}}\\
\text{ subject to }\forall \alpha\leq r \; \Expb{h_\beta(X)G\beta(X)\indicator{0\leq X\leq\alpha}}\geq 0 \\
\text{ and } \Expb{h_\beta(X)G\beta(X)\indicator{0\leq X\leq r}}= 0\;, \beta(r)=\beta(r^+)  
\end{gather*}
where $\beta(r^+)$ is given by the strategy that had reserve value at $r$. The continuity requirement is needed for Myerson's formula to apply as is, I think. 

Note that the constraints mean that the max revenue of the seller is achieved for the reserve value 0 and it is 0. We now that this is the case, because otherwise we could use thresholding below the reserve value to increase our revenue and not change that of the seller. So that guarantees that the reserve value is 0. (The revenue at $\alpha$ is the difference $\Expb{h_\beta(X)G\beta(X)\indicator{0\leq X\leq r}}-\Expb{h_\beta(X)G\beta(X)\indicator{0\leq X\leq\alpha}}$ so it's negative if $\beta$ is feasible for our problem.  )

The program is written in a slightly different fashion than in the text above to be in the same form as in \cite{TapiaTrossetKKTInfiniteDim94}, which maximizes a functional subject to constraints. 

Now the nice thing about the above formulation (maybe?) is that if we look at the computations we did above, we computed the variation of $F(\beta)$ by $\lim \frac{\partial F(\beta+t\rho)}{\partial t}$ and we ended up with something of the form 
$$
\lim_{t\tendsto 0} \frac{\partial F(\beta+t\rho)}{\partial t}=DF(\beta;\rho)=\Exp{\rho(X)M_\beta(X)+\rho'(X)W_\beta(X)}\;.
$$
Though note that we used integration by parts above...

So this operator is linear in $\rho$. To apply \cite{TapiaTrossetKKTInfiniteDim94} or a bunch of things, we need to check Fréchet differentiability. 

One big issue is what space to work in. We basically need $h_\beta$ to be well defined and integrable or square integrable and to be able to use integration by parts. So it's natural to look into Sobolev spaces. Natural ones seem to be $H^{1}$, which is a Hilbert space and $W^{1,1}$ which is Banach. Note that the $\norm{f}_{H^1}^2=\norm{f}^2_{L^2}+\norm{f'}^2_{L^{2}}$, even though $f'$ may have to be understood in a weak sense. So it's reasonable to try $\mathbf{H^1}$. 

If we look at $DF(\beta;\cdot)$ it is a linear operator. Furthermore, by Cauchy-Schwarz, 
$$
|DF(\beta;\rho)|\leq \norm{\rho}_{L^2}\norm{M_{\beta(X)}}_{L^2}+\norm{\rho'}_{L^2}\norm{W_{\beta(X)}}_{L^2}\leq \sqrt{2}\max(\norm{M_{\beta(X)}}_{L^2},\norm{W_{\beta(X)}}_{L^2})\norm{\rho}_{H^1}\;.
$$
So we may have Fréchet differentiability since this linear operator appears to be bounded continuous.

\subsection{Side notes}
These are just random notes to try to pinpoint possible problems and get at solutions... 
\subsubsection{How to transform an ``$L_2$'' gradient into an $H^1$ gradient}
When we computed the variation of the revenue of the seller at $r$ we ended up with a quantity of the form 
$$
I(\rho)=\int_a ^b h\rho + g \rho'=\int_a^b (h-g')\rho +g(b)\rho(b)-g(a)\rho(a)\;.
$$
We focused on the second formulation, as it was fairly natural for steepest/``gradient'' descent. And it looked like a gradient in $L_2$, using $h-g'$ as the vector of interest. Now one question is whether we can transform this into a gradient in $H^1$. 

Recall that 
$$
(\alpha,\rho)_{H^1}=\int \alpha\rho+\alpha'\rho'=\int(\alpha-\alpha^{''})\rho+\alpha'(b)\rho(b)-\alpha'(a)\rho(a)\;,
$$
if we assume that $\alpha$ has 2 derivatives. 

So the $H^1$ gradient associated with $I(\rho)$ could be defined as the function $\alpha$ such that 
$$
\begin{cases}
\alpha-\alpha"=h-g'\\
\alpha'(b)=g(b)\;, \text{ and } \alpha'(a)=g(a)\;.	
\end{cases}
$$
Note that the two independent solutions of $\alpha-\alpha"=0$ are $\alpha_\pm(x)=\exp(\pm x)$.
So 
$$
\alpha_{I(\rho)}=(A\exp(x)+B\exp(-x))+m(x)\;, m \text{ being a particular integral}
$$
A, B determined by edge conditions. Slides on the internet also give variational representation to connect $L_2$ and $H^1$ gradients. 
Practically, the particular integral would have to be determined numerically. And then we would use that to do gradient descent. Note that this amounts to finding the best $\rho$ to minimize $I(\rho)$. The gradient representation somehow makes this ``easy''. 

Note that if $I(\rho)=0$ for all $\rho$ in $H_1$, then $\alpha=0$, $h=g'$, $g(b)=g(a)=0$. So in our KKT having the first representation of $I(\rho)=\int_{a}^b (h-g')\rho+g(b)\rho(b)-g(a)\rho(a)$ may be enough to conclude. 
\subsection{Can we formulate the problem in $L_2$?}
Short answer is no.... 
Recall that the revenue of the seller is 
$$
R(\beta)=\int_a^b (\beta-\beta'(1-F)/f)G(\beta) f=\int_a^b [\beta f-(1-F)\beta']G(\beta)=
\int_a^b [\beta (F-1)]'G(\beta)
\;.
$$
Let's call $\Gamma$ a primitive of $G$ and interpret $\beta'G(\beta)$ as $\Gamma(\beta)'$. Then we can integrate by parts to get 
$$
R_{int}(\beta)=\int_a^b (\beta G(\beta)-\Gamma(\beta)) f-\left.(1-F)\Gamma(\beta)\right|_a^b\;.
$$
The possible advantage of this formulation is that it does not involve $\beta'$. So this might suggests that we could try to work with only continuous functions or something, though our integration by parts probably hid the fact that we were in $H^1$ or something like that. Also, as we'll see the need to do evaluations, i.e. calls to $\beta(b)$, $\beta(a)$ ruins the regularity in $L_2$. 

With this formulation, we can nonetheless easily compute the variation:
$$
\lim_{t\tendsto 0}\frac{\partial}{\partial t} R_{int}(\beta+t\rho)=
\int_a^b \rho(G(\beta)+\beta g(\beta)-G(\beta)) f-\left.(1-F)\rho g(\beta)\right|_a^b
=\int_a^b \rho \beta g(\beta) f-\left.(1-F)\rho g(\beta)\right|_a^b
$$
So we recover the results we had above but it might be slightly simpler, though it's still integration by parts. 

One hope of the $R_{int}$ formulation was that we could do gradient descent in $L_2$ with it. However, it's clear that as a function it is badly behaved in $L_2$ because the mapping $\rho\mapsto \rho(a)$ or $\rho(a)-\rho(b)$ is clearly not continuous in $L_2$. 

As we saw above (see also \cite{TapiaTrossetKKTInfiniteDim94} and I'm sure a bunch of references), it's well behaved in $H^1$. 

To be pedantic, the representation of the gradient as an element of the vector space works in a Hilbert space because of the Riesz representation theorem. That's sort of why we need the space to be complete/Hilbert, I guess.  



\subsection{Control formulation(??)}
One question is whether we can use a control formulation, which is quite classical actually in the calculus of variations (\cite{BertsekasControlBook2000,FlemingRishel75}).

The ``idea''  is to use $\psi$ or $h_\beta$ as control and $\beta$ as variable. Let's call $t$ our value. So $\psi_B(\beta(t))=\beta(t)-\beta'(t)\frac{1-F(t)}{f(t)}$. In his notation, $u(t)=x(t)-x'(t)\frac{1-F(t)}{f(t)}$.

To follow Bertsekas' notation, we have
$$
x'(t)=(x(t)-u(t))\lambda(t)\;, i.e. x'(t)=\mathfrak{f}(x(t),u(t),t)
$$
where $\lambda(t)=f(t)/(1-F(t))$ is the hazard rate. Note that he deals with the time dependent nature of the thingy by adding a dummy state variable $y(t)=t$. 
We may have to do backward control, i.e formulate everything in terms of $r-t$... So the initial condition would be $x(r-t)=\beta(r)$ for continuity. ok I have not done it. 

In the forward formulation, we seek to 
$$
\max_{u,x}\int_0^r (t-u(t))G(x(t))f(t) dt \text{ i.e. } \min_{u,x} \int_0^r (u(t)-t)G(x(t)) f(t) dt\;.
$$
The admissible controls satisfy 
$$
\forall r_0\leq r\;, \int_0^{r_0} u(t)G(x(t))f(t)dt \geq 0\;, \int_0^{r} u(t)G(x(t))f(t)dt = 0\;,
$$
or 
$$
\forall r_0\leq r\;, \int_{r_0}^{r} u(t)G(x(t))f(t)dt \leq 0\;, \int_0^{r} u(t)G(x(t))f(t)dt = 0\;,
$$
That way the max revenue of the seller is achieved for $r_0=0$. 




Not entirely clear if that falls into the standard control toolbox kind of thing because the admissibility constraints are a bit complicated... 

But would this give another approach to solving the problem?

\subsection{Another thing}

We note that the constraints can be written $\int_{r_0}^r (\beta (1-F))' G(\beta)\geq 0$ with equality at $r_0=0$. And we're trying to maximize under that constraint 
$$
\max \int_0^r xG(\beta(x))f(x)dx\;.
$$
If we call $\gamma=\beta(1-F)$, we have $\gamma\geq 0$. $\gamma/(1-F)$ increasing but let's forget about this. 
Then the optim problem is 
$$
\begin{cases}
\max_\gamma \int_0^ r x G(\gamma/(1-F))f(x)dx\;,\\
\text{subject to } \int_{r_0}^r	\gamma' G(\gamma/(1-F))\geq 0 \text{ and } \int_{0}^r	\gamma' G(\gamma/(1-F))= 0
\end{cases}
$$

With lot of manipulation optimality conditions at our solutions is starting to look like Gronwall. Though that might be due to a number of computational mistakes.

Meta question is whether our initial set of integral inequalities would imply something like the only feasible functions are less than $C/1-F(x)$ which would mean that we just took the pointwise max and so we'd be done...

Beside Gronwall (after integrating $\gamma$ by parts), a bunch of references point to work by Pachpatte. The Bihari-Lasalle inequality also seems vaguely related but it's not totally what we want... Though it seems that the question is very natural. A related issue is whether our solution is an isolated point of the feasible set but that seems hard to believe. That's the related in the general KKT to the issue of constraint qualifications, which is essentially as it guarantees strong duality. 

\subsection{The case $G(x)=\min(x,1)$}\label{subsec:app:particularCaseOptimality}
Let $r$ be given. Call $-h(x)$ the revenue of the seller on $[x,r]$. The constraints on $h$ is that $h(r)=0$, $h(0)=0$ and $h\geq 0$ on $[0,r]$. That way the revenue of the seller is maximized at $x^*=0$. 

We assume that $\beta\leq \beta(r)=r<1$. So then $G(\beta)=\beta$. 
\subsubsection{Preliminaries}
In differential form, our constraints can be written 
$$
\int_x^r [\beta(F-1)]' G(\beta)=\int_x^r [\beta(F-1)]'\beta= \int_x^r [\beta(F-1)]'\frac{\beta (F-1)}{F-1}=-h\;.
$$
So if $u=[\beta(1-F)]^2$, we have equivalently 
$$
\int_x^r u' \frac{1}{1-F}=2h(x)\;.
$$
If we integrate by parts, using the fact that $(1/(1-F))'=f/(1-F)^2$ and call $m(x)=u(x)/(1-F(x)=\beta^2(1-F)$, we get 
\begin{equation}\label{eq:definitionAuxiliaryFunctionm}
m(r)-m(x)-\int_x^r m(u)\frac{f(u)}{1-F(u)}=2h(x)\;.
\end{equation}
Assuming temporarily $h$ is differentiable, we differentiate Equation \eqref{eq:definitionAuxiliaryFunctionm} to get 
$$
-m'(x)+m(x)g(x)=2h'(x)\;, \text{ with } g(x)=\frac{f(x)}{1-F(x)}=-(\log(1-F))'\;.
$$
Because this is a first order ODE, we can integrate this equation fully to get 
$$
m(x)=\frac{1}{1-F(x)}\left[\beta^2(r)(1-F(r))^2+2\int_x^r h'(t)(1-F(t)) dt \right]\;.
$$
Note that this is the solutions among $m$ that are differentiable. 
\subsubsection{Key result}
So we have the following theorem. 
\begin{theorem}
Suppose $G(x)=x$ and call $-h$ the revenue of the seller at $x$. The unique shading function $\beta$ such that $\beta^(1-F)$ is differentiable and $\beta(x)\leq 1$ is $\beta>0$ such 
$$
\beta^2(x;h)=\beta^2(x)=\frac{1}{(1-F(x))^2} \left[\beta^2(r)(1-F(r))^2+2\left(\int_x^r h(t)f(t)dt - h(x)(1-F(x))\right) \right]\;.
$$		
Recall that $\beta^2(r)=r$. Of course $h=0$ corresponds to our thresholded function. 
\end{theorem}

\begin{proof}
Put all of the above together and then integrate by parts 	$\int_x^r h'(t)(1-F(t)) dt$ to get the formulation above. 
\end{proof}

\textbf{Remark~:} we see that $\beta^2_h$ depends linearly on $h$. So it suggests that if the optimum for our optim problem was achieved for $h\neq 0$, it would work for $\lambda h$, any $\lambda>0$. So we can do perturbative analysis at $h$ fixed, by looking at $\beta^2(\cdot;\eps h)$. 
\subsubsection{Back to our optim problem}
We wish to maximize 
$$
\Pi(h)=\int_0^r x G(\beta(x;h)) f(x) dx =\int_0^r x \beta(x;h) f(x) dx\;,
$$
as we assume that $\beta(x;h)$ remains below 1. 

Consider $\Pi(\eps h)$, with $\eps$ very small. Since $\sqrt{1+t}=1+\frac{t}{2}$, we see that 
$$
\beta(x;\eps h)=\beta(x;0)+\frac{\eps}{\beta(r)(1-F(r))}\frac{1}{1-F(x)}\left[\int_x^r h(t)f(t)dt-h(x)(1-F(x))\right]\;,
$$
where we have used that $h(r)=0$. So we have 
$$
\Pi(\eps h)=\Pi(0)+\frac{\eps}{\beta(r)(1-F(r))} \int_0^r \frac{xf(x)}{1-F(x)} \left[\int_x^r h(t)f(t)dt-h(x)(1-F(x))\right]dx\;.
$$
The question becomes whether 
$$
\boxed{
\int_0^r \frac{xf(x)}{1-F(x)} \left[\int_x^r h(t)f(t)dt-h(x)(1-F(x))\right]dx\leq 0\;.
}
$$
\begin{lemma}
Suppose that $\psi_F(x)=x-\frac{1-F(x)}{f(x)}\leq 0$ on $[0,r]$. Then, if $h\geq 0$, 
$$
\int_0^r \frac{xf(x)}{1-F(x)} \left[\int_x^r h(t)f(t)dt-h(x)(1-F(x))\right]dx\leq 0
$$	
\end{lemma}
\begin{proof}
We have, using Fubini's theorem,
\begin{align*}
\int_0^r \frac{xf(x)}{1-F(x)} \left[\int_x^r h(t)f(t)dt-h(x)(1-F(x))\right]dx&=-\int_0^r xh(x)f(x)+\int_0^r\int_0^r
\frac{xf(x)}{1-F(x)} h(t)f(t)\indicator{t>x} dx dt \;, \\
&=-\int_0^r xh(x)f(x)+\int_0^r
h(t)f(t) \int_0 ^x\frac{yf(y)}{1-F(y)}dy  dt\;,\\
&=-\int_0^r h(x)f(x)\left[x-\int_0 ^x\frac{yf(y)}{1-F(y)}dy\right]\;.
\end{align*}
Now since $\psi_F(x)=x-\frac{1-F(x)}{f(x)}\leq 0$, we have equivalently
$$
\frac{xf(x)}{1-F(x)}\leq 1\;.
$$
Hence, 
$$
\int_0 ^x\frac{yf(y)}{1-F(y)}dy\leq \int_0^x 1 dy =x\;. 
$$
We conclude that for all $h\geq 0$, 
$$
\int_0^r \frac{xf(x)}{1-F(x)} \left[\int_x^r h(t)f(t)dt-h(x)(1-F(x))\right]dx\leq 0\;.
$$
\end{proof}


We have the following theorem.
\begin{theorem}
For the problem of revenue optimization of the buyer, thresholding is a locally optimal when the competition has cdf $G(x)=\min(x,1)$ for $x\geq 0$. 

Furthermore, it is globally optimal among bidding strategies that are less than 1
\end{theorem}

\begin{proof}
The local optimally comes from the previous analysis. 

The global optimality comes from the fact that using the concavity of $\sqrt{1+x}$, we have $\sqrt{1+x}\leq 1+\frac{x}{2}$ for all $x\geq -1$. Then the upper bound is what we computed above. So an upper bound on the revenue is lower than the thresholded revenue and we have global optimality. 	
\end{proof}

\textbf{Remarks~:} this proof should work locally in many cases, as we would linearize $G$ around $\beta^*$ and find the family of admissible strategies through 1st order ODEs. And then the arguments should go through reasonably well. For global optimality, it is less clear. Fundamentally doing that is not that different from KKT. But we get a bit more information about the class of possible shading functions.  
\subsection{The general case, local optimality}\label{subsec:app:generalCaseOptimality}
It seems that there is a direct approach to local optimality using the same differential idea as above. 
Let $\eps>0$ and $\beta_\eps=\beta^*(1+\eps \rho)$. $\beta^*=C/(1-F(x))$ is the shading function corresponding to the thresholded. $C=r(1-F(r))$. $\rho$ is a function. We require $\rho(r)=0$ to have continuity of $\beta_\eps$ at $r$. 
Recall the constraints 
$$
\forall x\leq r\;,\;  \int_x^r [\beta(F-1)]' G(\beta)=-h(x)\leq 0 \;, \text{ and } h(0)=0\;.
$$
$h(r)=0$ by construction. Because $[\beta^*(F-1)]'=0$, we have 
$$
\int_x^r [\beta_\eps(F-1)]' G(\beta)=\eps \int_x^r (\rho\beta^*(F-1))' G(\beta^*+\eps \rho\beta^*)=-h_\eps
$$
and hence by limiting ourselves to the first order term in the Taylor expansion, 
$$
\int_x^r (\rho\beta^*(F-1))' G(\beta^*)=-h(x)\leq 0\;, \forall x\leq r\;.
$$
Assuming that $h$ is differentiable, we can differentiate the previous equality to get 
$$
(\rho(x)\beta^*(x)(F-1)(x))' G(\beta^*(x))=h'(x)\;,
$$
and using the fact that $\rho(r)=0$ because we want continuity at $r$, we get 
$$
\beta^*(x)\rho(x)(1-F(x))=\int_x^r \frac{h'(x)}{G(\beta^*(x))}dx=\int_x^r \frac{h(x)[\beta^{*}]'(x)g(\beta^*(x))}{G^2(\beta^*(x))}dx -\frac{h(x)}{G(\beta^*(x))}\;.
$$
The last equality comes from integration by parts. 

\subsubsection{Back to our optimization problem}
Recall that we see to maximize over admissible $\rho$'s (i.e. those for which the inequality constraints are verified), 
$$
\max_\rho \int_0^x x f(x) G(\beta^*(x)(1+\eps \rho(x))) dx\simeq \max_\rho \int_0^x x f(x) G(\beta^*(x))+ 
\eps \int_0^r x f(x) g(\beta^*(x)) \rho(x) \beta^*(x) dx\;.
$$
Where the equality is to first order in the Taylor expansion. 
We claim that if $\rho$ is admissible, then the second term is negative. 
\begin{lemma}
Let $\beta^*(x)=C/(1-F(x)$. Suppose that $\psi_F(x)\leq 0$ on $[0,r)$. Suppose the function $\rho$ is such that for $h\geq 0$, $h(r)=0$
$$
\beta^*(x)\rho(x)(1-F(x))=\int_x^r \frac{h(x)[\beta^{*}]'(x)g(\beta^*(x))}{G^2(\beta^*(x))}dx -\frac{h(x)}{G(\beta^*(x))}\;.
$$
Then 
$$
I=\int_0^r x f(x) g(\beta^*(x)) \rho(x) \beta^*(x) dx\leq 0\;.
$$
\end{lemma}
\begin{proof}
The strategy is the same as above. Let us call $\beta^*=\beta$ to make the notation less cumbersome. 
Replacing $\rho$ by its value, we have, using the fact that $\beta(x)=C/(1-F(x))$,
\begin{align*}
I/C&=-\int \frac{xf(x)}{1-F(x)}g(\beta(x)) \frac{h(x)}{G(\beta(x))} dx+\int_0^r dx \frac{xf(x)}{1-F(x)}g(\beta(x))\int_x^r \frac{h(t)\beta'(t)g(\beta(t))}{G^2(\beta(t))}dt\\
&=-\int \frac{xf(x)}{1-F(x)}g(\beta(x)) \frac{h(x)}{G(\beta(x))} dx+
\int_0^r\int_0^r \frac{xf(x)}{1-F(x)}g(\beta(x))\frac{h(t)\beta'(t)g(\beta(t))}{G^2(\beta(t))} \indicator{t\geq x} dx dt\\
&=-\int \frac{xf(x)}{1-F(x)}g(\beta(x)) \frac{h(x)}{G(\beta(x))} dx+
\int_0^r dx \frac{h(x)\beta'(x)g(\beta(x))}{G^2(\beta(x))} \int_0^x \frac{yf(y)}{1-F(y)}g(\beta(y))dy
\end{align*}
Now recall that $\beta'(t)=Cf/(1-F)^2$, $C>0$,  so that 
\begin{align*}
\int_0^x \frac{yf(y)}{1-F(y)}g(\beta(y))dy&=\frac{1}{C} \int_0^x y(1-F(y))\beta'(y)g(\beta(y))dy\;,\\
&=\frac{1}{C}\left[\left.t(1-F(t))G(\beta(t))\right|_0^x-\int_0^xG(\beta(t))[t(1-F(t))]' \right]\;.
\end{align*}
Of course, $(t(1-F(t)))'=-f(x)\psi_F(x)\geq 0$ since $\psi_F(x)\leq 0$. So we have 
$$
\int_0^x \frac{yf(y)}{1-F(y)}g(\beta(y))dy\leq \frac{1}{C} x (1-F(x)) G(\beta(x))\;.
$$
Hence, since $\beta'(x)>0$ and $h(x)>0$
\begin{align*}
\int_0^r dx \frac{h(x)\beta'(x)g(\beta(x))}{G^2(\beta(x))} \int_0^x \frac{yf(y)}{1-F(y)}g(\beta(y))dy
&\leq 
\int_0^r dx \frac{h(x)\beta'(x)g(\beta(x))}{G^2(\beta(x))} \frac{1}{C} x (1-F(x)) G(\beta(x))\\
&=\int_0^r dx \frac{h(x)\frac{Cf(x)}{[1-F(x)]^2}g(\beta(x))}{G(\beta(x))} \frac{1}{C} x (1-F(x))\\
&=\int_0^r dx \frac{xh(x)\frac{f(x)}{[1-F(x)]}g(\beta(x))}{G(\beta(x))}
\end{align*}
We conclude that 
$$
I\leq 0\;.
$$
\end{proof}
We have the following theorem. 
\begin{theorem}
Thresholding is locally optimal. 	
\end{theorem}
Proof: just put everything above together. 


==> splineStuffNEK.tex <==
\subsection{An attempt with first-order splines}
\label{splines_section}
A natural question is to ask whether the buyer can compute shading strategies directly numerically. For this it is natural to look back at the gradient of the bidder's utility in the direction of a certain function $\rho$. For bidder $i$, the directional derivative of this utility is by elementary calculus
\begin{align*}
\left.\frac{\partial}{\partial t} U_i(\beta_t)\right|_{t=0}&=\Expb{\left\{g(\beta(X_i))[X_i-\beta(X_i)]\right\}\rho(X_i)\indicator{X_i\geq x_\beta}}\\
&+G(\beta(x_{\beta}))\left[\frac{x_{\beta}f(x_{\beta})}{h_{\beta}^{'}(x_\beta)}-(1-F(x_{\beta}))\right]\rho(x_{\beta})\\
&-\frac{\rho'(x_{\beta})x_{\beta}(1-F(x_{\beta}))G(\beta(x_{\beta}))}{h_{\beta}^{'}(x_\beta)}\;.
\end{align*}

A natural idea is to expand the shading function in a basis, i.e. write 
$$
\beta(x)=\sum_{i=1}^N c_i(\beta) f_i(x)\;,
$$
and try to optimize over $c_i$. It would be even more natural to do a form of isotonic regression and optimize over non-decreasing functions directly; we will look at this later. 

\paragraph{A natural basis} Splines (see e.g. \cite{htfElementsStatLearning} for a practical introduction) are a natural candidate for the function $f_i$'s. In particular, first order splines are piecewise continuous functions, hence evaluating derivatives is trivial and it is easy to account in the formula above for the finitely many discontinuities of the derivative that will arise. If $\xi_k$'s are given knots, first order splines correspond to the functions 
$$
f_1=1, f_2(x)=x, f_{k+2}(x)=(x-\xi_k)_+=\max(x-\xi_k,0)\;.
$$
Higher order splines could of course also be used. 

\begin{lemma}
As described above, the optimal shading problem can be numerically approximated using steepest descent by a succession of linear programs, provided the non-decreasing constraint on $\beta$ can be written linearly in $c_i$. This of course the case for 1st order spline.
\end{lemma}
\begin{proof}
	Note that after the function is expanded in a basis, the functional gradient above becomes a standard gradient, and the bidder can improve their shading function by performing steepest descent. 	
If the reserve value is not one of the knots, the gradient above is easy to compute. At each step of the optimization one needs to solve a constrained LP to ensure that the solution is increasing. 

For 1st order splines, because the derivative is constant between knots, checking that for all $x$, $\beta'(x)\geq 0$ amounts to checking finitely many linear constraints and hence is amenable to an LP. 
\end{proof}

This approach amounts to an exploration of parts of the space of shading functions. Since the objective is not even continuous, though differentiable in a large part of the parameter space, the optimization problem is hard. In our experiments, we got significant improvement over bidding truthfully by using the above numerical method. However, wwe encountered the discontinuities of the optimization problem described above: our numerical optimizer got stuck at shading functions around which the reserve value was very unstable, which corresponds to revenue curves for the seller with several distant (approximate) local maxima: a small perturbation in function space does not induce much loss of the revenue on the seller side, but can have a huge impact on the reserve value and hence the buyer revenue. Note that in our numerical experiments we did not enforce the non-decreasing-constraint on $\beta$ but ended up with solutions that were non-decreasing. \redtext{Should we point to pictures?} 


Hence, in the next section, we introduce a relaxation of the problem which is easier to optimize and which has the same solutions as our initial objective. \redtext{DOUBLE CHECK THAT}. We also change the class of shading functions we consider and using neural networks to fit them. Before we describe these experiments we provide some theory for the problem of optimizing buyer revenue in lazy second price auctions. 

